Learning Nonlinear Loop Invariants with Gated Continuous Logic Networks (Extended Version)

Verifying real-world programs often requires inferring loop invariants with nonlinear constraints. This is especially true in programs that perform many numerical operations, such as control systems for avionics or industrial plants. Recently, data-driven methods for loop invariant inference have shown promise, especially on linear invariants. However, applying data-driven inference to nonlinear loop invariants is challenging due to the large numbers of and magnitudes of high-order terms, the potential for overfitting on a small number of samples, and the large space of possible inequality bounds. In this paper, we introduce a new neural architecture for general SMT learning, the Gated Continuous Logic Network (G-CLN), and apply it to nonlinear loop invariant learning. G-CLNs extend the Continuous Logic Network (CLN) architecture with gating units and dropout, which allow the model to robustly learn general invariants over large numbers of terms. To address overfitting that arises from finite program sampling, we introduce fractional sampling---a sound relaxation of loop semantics to continuous functions that facilitates unbounded sampling on real domain. We additionally design a new CLN activation function, the Piecewise Biased Quadratic Unit (PBQU), for naturally learning tight inequality bounds. We incorporate these methods into a nonlinear loop invariant inference system that can learn general nonlinear loop invariants. We evaluate our system on a benchmark of nonlinear loop invariants and show it solves 26 out of 27 problems, 3 more than prior work, with an average runtime of 53.3 seconds. We further demonstrate the generic learning ability of G-CLNs by solving all 124 problems in the linear Code2Inv benchmark. We also perform a quantitative stability evaluation and show G-CLNs have a convergence rate of $97.5\%$ on quadratic problems, a $39.2\%$ improvement over CLN models.

==> sections/edits.tex <==
\begin{comment}
1. Section 1 par 1, add sentence and reference to POPL17 paper
2. Section 2.1, rephrase the formulation of loop invariant
3. Section 2.2, state that we use product t-norm in implementation.
4. Section 2.3, sufficiently large $B$ and "sufficiently small" $\epsilon$
5. Section 4, reference arxiv version for proofs
6. Section 4.1 before Property 1, add coefficient extraction.
7. Section 4.2, address motivation and over-fitting of PBQU.
8. Section 4.3, change Figure 8c to double digit precision
9. Section 4.3, add pointer to new subsection in the end
10. Section 5.2.1, divide $\lambda$ into $\lambda_1$ and $\lambda_2$.
11. Section 5.4, new subsection on fractional sampling implementation
12. Section 6 in System Configuration, add z3 limitation.
13. Section 6 in System Configuration, add hyperparameters.
14. References, change cln2inv and si2019synthesizing to non-arxiv version



Todo
1. Inequality learning new implementation
2. An overview section (unlikely)
3. Check copyright, CCS concepts, and keywords


\end{comment}
